An architecture for enabling A/B experiments in automotive embedded software

A/B experimentation is a known technique for data-driven product development and has demonstrated its value in web-facing businesses. With the digitalisation of the automotive industry, the focus in the industry is shifting towards software. For automotive embedded software to continuously improve, A/B experimentation is considered an important technique. However, the adoption of such a technique is not without challenge. In this paper, we present an architecture to enable A/B testing in automotive embedded software. The design addresses challenges that are unique to the automotive industry in a systematic fashion. Going from hypothesis to practice, our architecture was also applied in practice for running online experiments on a considerable scale. Furthermore, a case study approach was used to compare our proposal with state-of-practice in the automotive industry. We found our architecture design to be relevant and applicable in the efforts of adopting continuous A/B experiments in automotive embedded software.

==> discussion.tex <==
\section{Discussion \label{discussion}}

\begin{table*}[h]
\normalsize
\caption{Papers selected which describing the architecture of A/B experiments, for web and embedded software.}
\begin{center}
{
\begin{tabular}{|p{0.03\textwidth}      p{0.55\textwidth}p{0.15\textwidth}p{0.05\textwidth}p{0.105\textwidth}|}
\hline
\textbf{No.} &
\textbf{Title of publication} & \textbf{Authors} & \textbf{Year} & \textbf{Environment} \\ \hline
P1 & Overlapping Experiment Infrastructure:
More, Better, Faster Experimentation \cite{google2010} & Tang \etal\ & 2010  & Web  \\ \hline
P2 & Architecture for Large-Scale Innovation Experiment Systems \cite{Eklund2012}  & Eklund \& Bosch & 2012 & Embedded \\ \hline
P3 & Eternal Embedded Software: Towards Innovation Experiment Systems \cite{Bosch2012} & Bosch \& Eklund & 2012 & Embedded  \\ \hline
P4 & Beyond data: from user information to business value through personalized recommendations and consumer science
 \cite{Amatriain2013} & Amatriain & 2013 & Web \\ \hline
P5 &  Online  controlled  experiments  at  large  scale \cite{Kohavi2013}  & Kohavi \etal\ & 2013 & Web  \\ \hline
P6 & Design  criteria  to  architect  continuous experimentation for self-driving  vehicles \cite{Giaimo2017} & Giaimo \& Berger & 2017 & Embedded \\ \hline
P7 & The RIGHT model for Continuous Experimentation \cite{Fagerholm2017} & Fagerholm \etal\ & 2017 & Web \\ \hline
P8 & Experimentation growth: Evolving trustworthy A/B testing capabilities in online software companies
\cite{Fabijan2018} & Fabijian \etal\ & 2018 & Web  \\ \hline
P9 & The Anatomy of a Large-Scale Experimentation Platform
\cite{Gupta2018} & Gupta \etal\ & 2018 & Web, app \& OS  \\ \hline
P10 & Scalable Data Reporting Platform for A/B Tests
\cite{Vasthimal2019} & Vasthimal \etal\ & 2019 & Web  \\ \hline
P11 & Experimentation in the Operating System: The Windows Experimentation Platform
\cite{Li2019} & Li \etal\ & 2019 & OS  \\ \hline
\end{tabular}}
\end{center}
\label{table_slr}
\end{table*}

In this paper, we presented a hybrid architecture combining in-vehicle and cloud elements that solves many problems in adopting continuous A/B experiments in automotive software.
Comparing to existing A/B experiment architecture for embedded software, our architecture offers the flexibility of being independent from a continuous deployment process.
By allowing parameter changes, the function can be experimented continuously without software changes.

However, we foresee some potential weakness in the design and they are discussed here.
Firstly, the threshold of functional behaviour change through parameters is low comparing to a complete software change.
The system enables A/B experiments for fine tuning of functions but not complete concept changes. 
In other words, the A/B testing can be done on relatively mature functions through our architecture.

Secondly, many parameters changes are not independent from each other in an automotive setting.
When multiple experiments are running simultaneously, the configuration of experiments becomes critical as suggested by \cite{google2010} and \cite{Kohavi2013} from their experience in the online businesses.
Similar to wed-facing applications, we need to consider contradicting parameters.
At the same time, some parameters configurations can be hierarchical when one function is deemed to be a sub-function of something else.
For instance, battery cooling temperature effects energy consumption management and climate comfort for the driver. 
This type of parameters adjustment needs to be coordinated when both functions are being A/B tested.
Performance of hierarchical functions cannot be determined individually. 
As a result, centralised, well-established and understood performance metrics need to be put in place before parallel/multiple experiments can be conducted simultaneously.

Thirdly, each team can independently determine parameters and observables.
Ideally, the teams shall coordinate their experiment designs when parameters or observables are shared in between different functions.
Such coordination requires organisational support \cite{Fabijan2018}.
As many automotive companies are going through agile transformation \cite{Mattos2020}, the data-driven development mindsets and support structure are gradually improving.
The speed of the transformation will influence how quickly an A/B experiment system can be put in place.

Fourthly, receiving cloud-based parameters requires an active internet connection that can be disrupted during a number of driving conditions, and usually has a delay in response.
Meanwhile the functions can be safeguarded through using local parameters as fallback, a function which requires millisecond response time cannot rely on cloud parameters.
Common examples of functions which are time critical include lane keeping assist, automatic breaking and active cruise control.
A possible setup for time critical functions is to embed the A and B versions of parameters in the software itself, and use the cloud to trigger the switch in between them.
As a trade-off, one will lose the freedom of tuning parameters independently from release processes.

Last but not least, some types of software are strictly governed by legal frameworks. 
Most types of legal requirements cover two dimensions.
First, functional changes can not demonstrate deteriorated performance in legal compliance tests. Second, vehicles cannot behave worse on the road in comparison to the lab tests.
We did not specifically address this issue in our software architecture, since legal compliance testing is built into software release processes in the industry.
Moreover, the potential performance change from cloud parameters can be demonstrated in advance if we limited the upper and lower limits of  parameters changes for all legally governed functions.

